UniFField: A Generalizable Unified Neural Feature Field for Visual, Semantic, and Spatial Uncertainties in Any Scene

Comprehensive visual, geometric, and semantic understanding of a 3D scene is crucial for successful execution of robotic tasks, especially in unstructured and complex environments. Additionally, to make robust decisions, it is necessary for the robot to evaluate the reliability of perceived information. While recent advances in 3D neural feature fields have enabled robots to leverage features from pretrained foundation models for tasks such as language-guided manipulation and navigation, existing methods suffer from two critical limitations: (i) they are typically scene-specific, and (ii) they lack the ability to model uncertainty in their predictions. We present UniFField, a unified uncertainty-aware neural feature field that combines visual, semantic, and geometric features in a single generalizable representation while also predicting uncertainty in each modality. Our approach, which can be applied zero shot to any new environment, incrementally integrates RGB-D images into our voxel-based feature representation as the robot explores the scene, simultaneously updating uncertainty estimation. We evaluate our uncertainty estimations to accurately describe the model prediction errors in scene reconstruction and semantic feature prediction. Furthermore, we successfully leverage our feature predictions and their respective uncertainty for an active object search task using a mobile manipulator robot, demonstrating the capability for robust decision-making.

==> tables/metrics_uncert.tex <==
\begin{table*}[ht]  % \textcolor{gray}{$0.0$}
    \centering
    %\captionsetup{justification=centering}
    \caption[Uncertainty evaluation]{\textbf{Uncertainty evaluation}. We compare our predicted uncertainties on the ScanNet dataset against dropout ensemble-based and random uncertainties of different modalities with the corresponding prediction error. For the correlation coefficient $\rho$, we additionally report the proportion of statistically significant correlation tests. %Predicted uncertainty generally outperforms dropout-based uncertainty across all error and uncertainty metrics, indicating a moderate correlation. The \gls{MAE} describes semantic uncertainty best.
    }
    \scalebox{1.}{
        \begin{tabular}{c|c|cc|ccc|ccc} \toprule
            \multirow{2}{*}{Space} & \multirow{2}{*}{Prediction Error} & \multicolumn{2}{c|}{\multirow{2}{*}{Uncertainty}} &   \multicolumn{3}{c|}{{AUSE} $\downarrow$} & \multicolumn{3}{c}{Correlation $\rho \uparrow$ (Significance $\uparrow$)} \\ \cline{5-7} \cline{8-10} %\hline
            & &  &  &  {{MAE}} & {{MSE}} & {{RMSE}} & {{MAE}} & {{MSE}} & {{RMSE}} \\ \hline
            \multirow{3}{*}{2D} & \multirow{3}{*}{Color} &\multirow{3}{*}{Visual} & Pred.    &    \textbf{0.213}  &  \textbf{0.243}  &  \textbf{0.233}  &  \textbf{0.474}  (0.97)  &  \textbf{0.481}  (0.97)  &  \textbf{0.481}  (0.97)  \\
                                  & &  & Drop.      &   0.263  &  0.310  &  0.289  &  0.375  (0.93)  &  0.380  (0.94)  &  0.380  (0.94)  \\
                                  & &     & Rand.       &   0.526  &  0.745  &  0.566  &  0.000  (0.04)  &  0.000  (0.04)  &  0.000  (0.04)   \\ \hline
                                       
            \multirow{3}{*}{2D} & \multirow{3}{*}{CLIP Feature} & \multirow{3}{*}{Semantic} & Pred.   &    \textbf{0.095}  &  \textbf{0.156}  &  \textbf{0.095}  &  \textbf{0.220}  (0.98)  &  \textbf{0.209}  (0.97)  &  \textbf{0.209}  (0.97)  \\
                                   & &  & Drop.    &   0.144  &  0.211  &  0.127  &  0.063  (0.54)  &  0.052  (0.54)  &  0.052  (0.54)  \\
                                   & &   & Rand.   &   0.170  &  0.238  &  0.141  &  0.000  (0.04)  &  0.001  (0.05)  &  0.001  (0.05)  \\ \hline

            % All voxels
            \multirow{3}{*}{3D} & \multirow{3}{*}{TSDF} & \multirow{3}{*}{Spatial}       & Pred.   &    \textbf{0.013}  &  \textbf{0.011}  &  \textbf{0.054}  &  0.561  (1.00)  &  0.561  (1.00)  &  0.561  (1.00)   \\
                               & &  & Drop.   &   0.164  &  0.184  &  0.326  &  \textbf{0.592}  (1.00)  &  \textbf{0.592}  (1.00)  &  \textbf{0.592}  (1.00)   \\
                               & &    & Rand.   &   0.965  &  0.967  &  0.969  &  0.000  (0.05)  &  0.000  (0.05)  &  0.000  (0.05)   \\ \bottomrule

        %    % Observed Voxels
        %    \multirow{2}{*}{TSDF} & \multirow{2}{*}{Spatial}   & Pred.   &    \textbf{0.045}  &  \textbf{0.048}  &  \textbf{0.097}  &  \textbf{0.841}  (1.00)  &  \textbf{0.841}  (1.00)  &  \textbf{0.841}  (1.00)   \\
        %                       &   & Drop.    &  0.159  &  0.150  &  0.266  &  0.817  (1.00)  &  0.817  (1.00)  &  0.817  (1.00)   \\ \bottomrule
        %                           %& Rand.   & Y &   0.856  &  0.901  &  0.854  &  0.000  (0.03)  &  0.000  (0.03)  &  0.000  (0.03)  \\  \bottomrule
    \end{tabular}
    }
    %\vspace{-1em}
    \label{tab:metrics_uncert_2d_rgb}
\end{table*}

% v1:
% \begin{table*}[ht]  % \textcolor{gray}{$0.0$}
%     \centering
%     \scalebox{1.0}{
%         \begin{tabular}{cc|ccc|ccc} \toprule
%             \multicolumn{2}{c|}{Uncertainty} & \multicolumn{3}{c|}{{AUSE} $\downarrow$} & \multicolumn{3}{c}{Correlation $\rho \uparrow$ (Signif. $\uparrow$)} \\ \hline
%             \multicolumn{1}{c}{Modality} & Method & {{MAE}} & {{MSE}} & {{RMSE}} & {{MAE}} & {{MSE}} & {{RMSE}} \\ \hline
%             \multirow{2}{*}{2D Visual} & Pred.      &  \textbf{0.213}  &  \textbf{0.243}  &  \textbf{0.233}  &  \textbf{0.474}  (0.97)  &  \textbf{0.481}  (0.97)  &  \textbf{0.481}  (0.97)  \\
%                                        & Drop.      &  0.263  &  0.310  &  0.289  &  0.375  (0.93)  &  0.380  (0.94)  &  0.380  (0.94)  \\ \hline
%                                        %& Rand.      &  0.526  &  0.745  &  0.566  &  0.000  (0.04)  &  0.000  (0.04)  &  0.000  (0.04)   \\ \hline
                                       
%             \multirow{2}{*}{2D Semantic} & Pred.   &  \textbf{0.095}  &  \textbf{0.156}  &  \textbf{0.095}  &  \textbf{0.220}  (0.98)  &  \textbf{0.209}  (0.97)  &  \textbf{0.209}  (0.97)  \\
%                                       & Drop.   &  0.144  &  0.211  &  0.127  &  0.063  (0.54)  &  0.052  (0.54)  &  0.052  (0.54)  \\ \hline
%                                       %& Rand.   &  0.170  &  0.238  &  0.141  &  0.000  (0.04)  &  0.001  (0.05)  &  0.001  (0.05)  \\ \hline

%             % All voxels
%             \multirow{2}{*}{3D Spatial}       & Pred.   &  \textbf{0.013}  &  \textbf{0.011}  &  \textbf{0.054}  &  0.561  (1.00)  &  0.561  (1.00)  &  0.561  (1.00)   \\
%                                    & Drop.   &  0.164  &  0.184  &  0.326  &  \textbf{0.592}  (1.00)  &  \textbf{0.592}  (1.00)  &  \textbf{0.592}  (1.00)   \\ \hline
%                                    %& Rand.   &  0.965  &  0.967  &  0.969  &  0.000  (0.05)  &  0.000  (0.05)  &  0.000  (0.05)   \\ \hline

%             % Observed Voxels
%             \multirow{2}{*}{3D Spatial}   & Pred.   &  \textbf{0.045}  &  \textbf{0.048}  &  \textbf{0.097}  &  \textbf{0.841}  (1.00)  &  \textbf{0.841}  (1.00)  &  \textbf{0.841}  (1.00)   \\
%                                    & Drop.   &  0.159  &  0.150  &  0.266  &  0.817  (1.00)  &  0.817  (1.00)  &  0.817  (1.00)   \\ \bottomrule
%                                    %& Rand.   &  0.856  &  0.901  &  0.854  &  0.000  (0.03)  &  0.000  (0.03)  &  0.000  (0.03)  \\  \bottomrule
%     \end{tabular}
%     }
%     %\captionsetup{justification=centering}
%     \caption[Uncertainty Metrics for Evaluating Visual Uncertainty]{\textbf{Uncertainty Metrics for Evaluating Visual Uncertainty}. We compare predicted (Pred.), dropout-based (Drop.), and random (Rand.) uncertainties with the color error using the error metrics $\varepsilon$ to evaluate their relationship, using both per-frame and per-scene strategies. For the correlation coefficient $\rho$, the significance consistency (Signif.) is reported additionally. Predicted uncertainty generally outperforms dropout-based uncertainty across all error and uncertainty metrics, indicating a moderate correlation.
%     %The quality of the uncertainty estimates is slightly improved when evaluating uncertainty per scene compared to per frame.
%     The \gls{MAE} describes semantic uncertainty best.}
%     \label{tab:metrics_uncert_2d_rgb}
% \end{table*}


% % v2:
% \begin{table*}[ht]  % \textcolor{gray}{$0.0$}
%     \centering
%     \scalebox{1.0}{
%         \begin{tabular}{cc|c|ccc|ccc} \toprule
%             \multicolumn{2}{c|}{Uncertainty} & Error &  \multicolumn{3}{c|}{{AUSE} $\downarrow$} & \multicolumn{3}{c}{Correlation $\rho \uparrow$ (Signif. $\uparrow$)} \\ \hline
%             \multicolumn{1}{c}{Modality} & Method & Type &  {{MAE}} & {{MSE}} & {{RMSE}} & {{MAE}} & {{MSE}} & {{RMSE}} \\ \hline
%             \multirow{2}{*}{2D Visual} & Pred.    & \multirow{2}{*}{Color} &   \textbf{0.213}  &  \textbf{0.243}  &  \textbf{0.233}  &  \textbf{0.474}  (0.97)  &  \textbf{0.481}  (0.97)  &  \textbf{0.481}  (0.97)  \\
%                                    & Drop.      &   &   0.263  &  0.310  &  0.289  &  0.375  (0.93)  &  0.380  (0.94)  &  0.380  (0.94)  \\ \hline
%                                        %& Rand.      & Y &   0.526  &  0.745  &  0.566  &  0.000  (0.04)  &  0.000  (0.04)  &  0.000  (0.04)   \\ \hline
                                       
%             \multirow{2}{*}{2D Semantic} & Pred.   & \multirow{2}{*}{Feature} &   \textbf{0.095}  &  \textbf{0.156}  &  \textbf{0.095}  &  \textbf{0.220}  (0.98)  &  \textbf{0.209}  (0.97)  &  \textbf{0.209}  (0.97)  \\
%                                    & Drop.   &   &   0.144  &  0.211  &  0.127  &  0.063  (0.54)  &  0.052  (0.54)  &  0.052  (0.54)  \\ \hline
%                                       %& Rand.   & Y &   0.170  &  0.238  &  0.141  &  0.000  (0.04)  &  0.001  (0.05)  &  0.001  (0.05)  \\ \hline

%             % All voxels
%             \multirow{2}{*}{3D Spatial}       & Pred.   & \multirow{2}{*}{TSDF} &   \textbf{0.013}  &  \textbf{0.011}  &  \textbf{0.054}  &  0.561  (1.00)  &  0.561  (1.00)  &  0.561  (1.00)   \\
%                                & Drop.   &  &   0.164  &  0.184  &  0.326  &  \textbf{0.592}  (1.00)  &  \textbf{0.592}  (1.00)  &  \textbf{0.592}  (1.00)   \\ \hline
%                                    %& Rand.   & Y &   0.965  &  0.967  &  0.969  &  0.000  (0.05)  &  0.000  (0.05)  &  0.000  (0.05)   \\ \hline

%             % Observed Voxels
%             \multirow{2}{*}{3D Spatial}   & Pred.   & \multirow{2}{*}{TSDF} &   \textbf{0.045}  &  \textbf{0.048}  &  \textbf{0.097}  &  \textbf{0.841}  (1.00)  &  \textbf{0.841}  (1.00)  &  \textbf{0.841}  (1.00)   \\
%                                & Drop.   &   &  0.159  &  0.150  &  0.266  &  0.817  (1.00)  &  0.817  (1.00)  &  0.817  (1.00)   \\ \bottomrule
%                                    %& Rand.   & Y &   0.856  &  0.901  &  0.854  &  0.000  (0.03)  &  0.000  (0.03)  &  0.000  (0.03)  \\  \bottomrule
%     \end{tabular}
%     }
%     %\captionsetup{justification=centering}
%     \caption[Uncertainty Metrics for Evaluating Visual Uncertainty]{\textbf{Uncertainty Metrics for Evaluating Visual Uncertainty}. We compare predicted (Pred.), dropout-based (Drop.), and random (Rand.) uncertainties with the color error using the error metrics $\varepsilon$ to evaluate their relationship, using both per-frame and per-scene strategies. For the correlation coefficient $\rho$, the significance consistency (Signif.) is reported additionally. Predicted uncertainty generally outperforms dropout-based uncertainty across all error and uncertainty metrics, indicating a moderate correlation.
%     %The quality of the uncertainty estimates is slightly improved when evaluating uncertainty per scene compared to per frame.
%     The \gls{MAE} describes semantic uncertainty best.}
%     \label{tab:metrics_uncert_2d_rgb}
% \end{table*}


% v3
% \begin{table*}[ht]  % \textcolor{gray}{$0.0$}
%     \centering
%     \scalebox{1.0}{
%         \begin{tabular}{cc|c|ccc|ccc} \toprule
%             \multicolumn{2}{c|}{\multirow{2}{*}{Uncertainty}} & \multirow{2}{*}{Error} &  \multicolumn{3}{c|}{{AUSE} $\downarrow$} & \multicolumn{3}{c}{Correlation $\rho \uparrow$ (Signif. $\uparrow$)} \\ \cline{4-6} \cline{7-9} %\hline
%             \multicolumn{1}{c}{Modality} & Method &  &  {{MAE}} & {{MSE}} & {{RMSE}} & {{MAE}} & {{MSE}} & {{RMSE}} \\ \hline
%             \multirow{2}{*}{2D Visual} & Pred.    & \multirow{2}{*}{Color} &   \textbf{0.213}  &  \textbf{0.243}  &  \textbf{0.233}  &  \textbf{0.474}  (0.97)  &  \textbf{0.481}  (0.97)  &  \textbf{0.481}  (0.97)  \\
%                                    & Drop.      &   &   0.263  &  0.310  &  0.289  &  0.375  (0.93)  &  0.380  (0.94)  &  0.380  (0.94)  \\ \hline
%                                        %& Rand.      & Y &   0.526  &  0.745  &  0.566  &  0.000  (0.04)  &  0.000  (0.04)  &  0.000  (0.04)   \\ \hline
                                       
%             \multirow{2}{*}{2D Semantic} & Pred.   & \multirow{2}{*}{Feature} &   \textbf{0.095}  &  \textbf{0.156}  &  \textbf{0.095}  &  \textbf{0.220}  (0.98)  &  \textbf{0.209}  (0.97)  &  \textbf{0.209}  (0.97)  \\
%                                    & Drop.   &   &   0.144  &  0.211  &  0.127  &  0.063  (0.54)  &  0.052  (0.54)  &  0.052  (0.54)  \\ \hline
%                                       %& Rand.   & Y &   0.170  &  0.238  &  0.141  &  0.000  (0.04)  &  0.001  (0.05)  &  0.001  (0.05)  \\ \hline

%             % All voxels
%             \multirow{2}{*}{3D Spatial}       & Pred.   & \multirow{2}{*}{TSDF} &   \textbf{0.013}  &  \textbf{0.011}  &  \textbf{0.054}  &  0.561  (1.00)  &  0.561  (1.00)  &  0.561  (1.00)   \\
%                                & Drop.   &  &   0.164  &  0.184  &  0.326  &  \textbf{0.592}  (1.00)  &  \textbf{0.592}  (1.00)  &  \textbf{0.592}  (1.00)   \\ \hline
%                                    %& Rand.   & Y &   0.965  &  0.967  &  0.969  &  0.000  (0.05)  &  0.000  (0.05)  &  0.000  (0.05)   \\ \hline

%             % Observed Voxels
%             \multirow{2}{*}{3D Spatial}   & Pred.   & \multirow{2}{*}{TSDF} &   \textbf{0.045}  &  \textbf{0.048}  &  \textbf{0.097}  &  \textbf{0.841}  (1.00)  &  \textbf{0.841}  (1.00)  &  \textbf{0.841}  (1.00)   \\
%                                & Drop.   &   &  0.159  &  0.150  &  0.266  &  0.817  (1.00)  &  0.817  (1.00)  &  0.817  (1.00)   \\ \bottomrule
%                                    %& Rand.   & Y &   0.856  &  0.901  &  0.854  &  0.000  (0.03)  &  0.000  (0.03)  &  0.000  (0.03)  \\  \bottomrule
%     \end{tabular}
%     }
%     %\captionsetup{justification=centering}
%     \caption[Uncertainty Metrics for Evaluating Visual Uncertainty]{\textbf{Uncertainty Metrics for Evaluating Visual Uncertainty}. We compare predicted (Pred.), dropout-based (Drop.), and random (Rand.) uncertainties with the color error using the error metrics $\varepsilon$ to evaluate their relationship, using both per-frame and per-scene strategies. For the correlation coefficient $\rho$, the significance consistency (Signif.) is reported additionally. Predicted uncertainty generally outperforms dropout-based uncertainty across all error and uncertainty metrics, indicating a moderate correlation.
%     %The quality of the uncertainty estimates is slightly improved when evaluating uncertainty per scene compared to per frame.
%     The \gls{MAE} describes semantic uncertainty best.}
%     \label{tab:metrics_uncert_2d_rgb}
% \end{table*}



% v4
% \begin{table*}[ht]  % \textcolor{gray}{$0.0$}
%     \centering
%     \scalebox{1.0}{
%         \begin{tabular}{cc|c|ccc|ccc} \toprule
%             \multicolumn{2}{c|}{\multirow{2}{*}{Uncertainty}} & \multirow{2}{*}{Error} &  \multicolumn{3}{c|}{{AUSE} $\downarrow$} & \multicolumn{3}{c}{Correlation $\rho \uparrow$ (Signif. $\uparrow$)} \\ \cline{4-6} \cline{7-9} %\hline
%              &  &  &  {{MAE}} & {{MSE}} & {{RMSE}} & {{MAE}} & {{MSE}} & {{RMSE}} \\ \hline
%             \multirow{2}{*}{2D Visual} & Pred.    & \multirow{2}{*}{Color} &   \textbf{0.213}  &  \textbf{0.243}  &  \textbf{0.233}  &  \textbf{0.474}  (0.97)  &  \textbf{0.481}  (0.97)  &  \textbf{0.481}  (0.97)  \\
%                                    & Drop.      &   &   0.263  &  0.310  &  0.289  &  0.375  (0.93)  &  0.380  (0.94)  &  0.380  (0.94)  \\ \hline
%                                        %& Rand.      & Y &   0.526  &  0.745  &  0.566  &  0.000  (0.04)  &  0.000  (0.04)  &  0.000  (0.04)   \\ \hline
                                       
%             \multirow{2}{*}{2D Semantic} & Pred.   & \multirow{2}{*}{Feature} &   \textbf{0.095}  &  \textbf{0.156}  &  \textbf{0.095}  &  \textbf{0.220}  (0.98)  &  \textbf{0.209}  (0.97)  &  \textbf{0.209}  (0.97)  \\
%                                    & Drop.   &   &   0.144  &  0.211  &  0.127  &  0.063  (0.54)  &  0.052  (0.54)  &  0.052  (0.54)  \\ \hline
%                                       %& Rand.   & Y &   0.170  &  0.238  &  0.141  &  0.000  (0.04)  &  0.001  (0.05)  &  0.001  (0.05)  \\ \hline

%             % All voxels
%             \multirow{2}{*}{3D Spatial}       & Pred.   & \multirow{2}{*}{TSDF} &   \textbf{0.013}  &  \textbf{0.011}  &  \textbf{0.054}  &  0.561  (1.00)  &  0.561  (1.00)  &  0.561  (1.00)   \\
%                                & Drop.   &  &   0.164  &  0.184  &  0.326  &  \textbf{0.592}  (1.00)  &  \textbf{0.592}  (1.00)  &  \textbf{0.592}  (1.00)   \\ \hline
%                                    %& Rand.   & Y &   0.965  &  0.967  &  0.969  &  0.000  (0.05)  &  0.000  (0.05)  &  0.000  (0.05)   \\ \hline

%             % Observed Voxels
%             \multirow{2}{*}{3D Spatial}   & Pred.   & \multirow{2}{*}{TSDF} &   \textbf{0.045}  &  \textbf{0.048}  &  \textbf{0.097}  &  \textbf{0.841}  (1.00)  &  \textbf{0.841}  (1.00)  &  \textbf{0.841}  (1.00)   \\
%                                & Drop.   &   &  0.159  &  0.150  &  0.266  &  0.817  (1.00)  &  0.817  (1.00)  &  0.817  (1.00)   \\ \bottomrule
%                                    %& Rand.   & Y &   0.856  &  0.901  &  0.854  &  0.000  (0.03)  &  0.000  (0.03)  &  0.000  (0.03)  \\  \bottomrule
%     \end{tabular}
%     }
%     %\captionsetup{justification=centering}
%     \caption[Uncertainty Metrics for Evaluating Visual Uncertainty]{\textbf{Uncertainty Metrics for Evaluating Visual Uncertainty}. We compare predicted (Pred.), dropout-based (Drop.), and random (Rand.) uncertainties with the color error using the error metrics $\varepsilon$ to evaluate their relationship, using both per-frame and per-scene strategies. For the correlation coefficient $\rho$, the significance consistency (Signif.) is reported additionally. Predicted uncertainty generally outperforms dropout-based uncertainty across all error and uncertainty metrics, indicating a moderate correlation.
%     %The quality of the uncertainty estimates is slightly improved when evaluating uncertainty per scene compared to per frame.
%     The \gls{MAE} describes semantic uncertainty best.}
%     \label{tab:metrics_uncert_2d_rgb}
% \end{table*}

